Which of These Best Describes Multiple Choice Evaluation with LLMs? A) Forced B) Flawed C) Fixable D) All of the Above

Multiple choice question answering (MCQA) is popular for LLM evaluation due to its simplicity and human-like testing, but we argue for its reform. We first reveal flaws in MCQA's format, as it struggles to: 1) test generation/subjectivity; 2) match LLM use cases; and 3) fully test knowledge. We instead advocate for generative formats based on human testing, where LLMs construct and explain answers, better capturing user needs and knowledge while remaining easy to score. We then show even when MCQA is a useful format, its datasets suffer from: leakage; unanswerability; shortcuts; and saturation. In each issue, we give fixes from education, like rubrics to guide MCQ writing; scoring methods to bridle guessing; and Item Response Theory to build harder MCQs. Lastly, we discuss LLM errors in MCQA, robustness, biases, and unfaithful explanations, showing how our prior solutions better measure or address these issues. While we do not need to desert MCQA, we encourage more efforts in refining the task based on educational testing, advancing evaluations.

==> 2025_acl_mcqa_sucks/pages/00_abstract.tex <==
\begin{abstract} {
Multiple choice question answering (\mcqa) is popular for LLM evaluation due to its simplicity and human-like testing, but we argue for its reform.
%
We first reveal flaws in~\mcqa's format, as it struggles to: 1) test generation/subjectivity; 2) match LLM use cases; and 3) fully~test knowledge.
%
We instead advocate for generative formats based on human testing---where LLMs construct
and explain answers---better~capturing user needs and knowledge while remaining easy to score.
We then show even when \mcqa is a useful format, its datasets suffer from: leakage; unanswerability; shortcuts; and saturation.
In each issue, we give fixes from education, like rubrics to guide MCQ writing; scoring methods to bridle guessing; and Item Response Theory to build harder MCQs.
Lastly, we discuss LLM errors in \mcqa---robustness, biases, and unfaithful explanations---showing how our prior solutions better measure or address these issues.
While we do not need to desert \mcqa, we encourage more efforts in refining the task based on educational testing, advancing evaluations.
}
\end{abstract}


==> 2025_acl_mcqa_sucks/pages/10_intro.tex <==
\section{Questioning Multiple Choice Questions}

Multiple choice question answering (\mcqa) is~the standard for large language model (LLM) evaluations, prized for simplicity and
similarity to human testing \cite{robinson2023leveraging}.
%
When designing new benchmarks, \mcqa seems easy to~implement
\cite{guo2023evaluating}, and when selecting new LLMs to use, \mcqa
leaderboards inform our decisions \cite{open-llm-leaderboard-v2}.
%
If you want to build a popular dataset, prove your LLM is smart,
or even publish a position paper, it is hard to avoid~\mcqa.

Standardized testing groups have long explored ways to
better use \mcqa for student testing \cite{angoff1971college}.
But despite years of use in \abr{nlp}~\cite{turney2003combining}, few have asked: 1) should \mcqa be a standard model evaluation format; and 2) are its datasets well-designed?
This position paper argues: \textbf{Evaluating LLMs with \mcqa has flaws in both its inherent format and dataset construction.}
We state our position in three points (Fig~\ref{fig:intro}).

\input{figures/intro}

We first argue \mcqa is not an ideal standardized format for LLM evaluations, showing its goal of ``pick the
best answer'' cannot optimally test generation or subjectivity
(\cref{subsection:best_answer}), misaligns with LLM use cases
(\cref{subsection:use_cases}), and poorly tests knowledge
(\cref{subsection:testing_what}).
Drawing from education, we advocate two \textit{generative}
improvements to \mcqa's format for future exploration: 1) providing
short, constructed-response answers without using choices
(\cref{subsection:constructed_response}); and 2) evaluating
explanations for model answers (\cref{subsection:justified_mcqa}).
%
These formats capture generation or subjectivity, match LLM use cases,
and improve knowledge testing, all while mostly preserving \mcqa's
simple scoring.


Next, we argue even when \mcqa is a useful format, its datasets suffer from: dataset leakage
(\cref{subsection:test_set_leakage}), unanswerable \mcq{}s~(\cref{subsection:quality}), shortcuts (\cref{subsection:artifacts}),
and saturation (\cref{subsection:saturation}), degrading \mcqa's utility.
%
To enhance \abr{nlp} dataset design, we offer solutions for each issue based on best practices in human
testing, like rubrics to flag \mcq errors (\cref{subsection:quality}),
metrics~to curb guessing from shortcuts
(\cref{subsubsection:shortcut_scoring}), and Item Response Theory
\cite{baker2001basics} to cull shoddy MCQs and make the ones left
more challenging~(\cref{subsection:irt}).

Lastly, we show many errors of LLMs in \mcqa directly relate to
\mcqa's flaws (\cref{section:models}).
%
These issues, like brittleness to perturbations
(\cref{subsection:robustness}), bias toward certain options, cultures,
and languages (\cref{subsection:bias}), and generating
unfaithful explanations (\cref{subsection:explanations}), can all be
better measured or addressed with our proposed improvements to \mcqa's
format and datasets.


Many promising improvements to \mcqa draw from education, a field dedicated to effective assessment
\cite{haladyna2002review}, but these practices are rarely used in \abr{nlp}.
Adopting them demands more effort---\mcqa{} is popular
as it seems simple---but this effort is worth it to improve
evaluations.
%
To encourage researchers to take on these challenges, we conclude with
guidelines for designing meaningful evaluations whether or not you use
\mcqa{}~(\cref{section:conclusion}).



==> 2025_acl_mcqa_sucks/pages/30_format.tex <==
\section{\mcqa is Flawed as a Standard Format} \label{section:format}

\mcqa is a simple format for student testing, but educators find
tradeoffs: it may not predict student success~\cite{moneta2017limitations} or assess knowledge~\cite{simkin2005multiple}.
%
We argue the same issues apply to \abr{nlp} and thus, \mcqa should not be considered a gold standard for evaluating LLMs.
Specifically, we show \mcqa's rigid goal
(\cref{subsection:best_answer}), misalignment with real LLM use
cases (\cref{subsection:use_cases}), and limited testing of knowledge~(\cref{subsection:testing_what}).

\input{figures/subjective}

\subsection{``\underline{Pick} the \textit{Best} Answer'' is Too Rigid} \label{subsection:best_answer}

One of \mcqa's key issues is its rigid goal: pick the best answer from a set of choices.
While easy to score, both designs---the use of
1) one gold answer; and 2) input choices---limit \mcqa's applicability.

First, one gold answer hinders \mcqa's use for evaluating subjectivity
\cite{finetti1965methods}.
Still, we use this format for commonsense \cite{bisk2020piqa}, morals \cite{yu-etal-2024-cmoraleval, scherrer2023evaluating}, and culture (\cref{subsection:bias}), where many choices can be~subjectively right (Figure~\ref{fig:subjective}).
\citet{Palta2024PlausiblyPQ} find~users rate distractors in commonsense MCQs as the most plausible choice in over 20\% of cases.
Thus, extra care is needed to write MCQs for subjective tasks.

Second, picking from choices means MCQs test \textit{validation}, useful in tasks
like LLM-as-a-judge or re-ranking which must compare answers
\cite{gu2024survey}, but inhibiting tasks like writing and coding that
require \textit{generation} \cite{celikyilmaz2020evaluation}.
%
One may argue \mcqa proxies generation (if you pick good answers, you generate good ones), but LLMs~lack validation/generation consistency
\cite{li2024benchmarking, west2023generative, balepur-etal-2025-reverse}.
%
Validation and generation are thus separate skills, so \mcqa is a poor format for evaluating generation ability.

In all, \mcqa best tests LLMs in objective validation, struggling with subjectivity and generation.

\subsection{Users Rarely Ask LLMs to Solve MCQs} \label{subsection:use_cases}

Many leaderboards aim to rank LLMs by their overall abilities, helping users select the best model for their needs \cite{xia2024top}.
Hence, they should adopt tasks that mirror the popularity of user needs, giving higher ranks to models that can actually help users \cite{balepur-etal-2024-smart, mozannar2025the}.

\mcqa is over-represented versus how LLMs are used; 32\% of the tasks in HELM
\cite{perlitz2023efficient}, 71\% in GPT-4's card \cite{achiam2023gpt}, and 79\% in OpenLLM (Big Bench has 21 \mcqa tasks) \cite{open-llm-leaderboard-v2} are \mcqa.
%
In contrast, \citet{ouyang2023shifted} find in ShareGPT's dataset of ChatGPT queries that nearly all user queries
ask for free-form text; we estimate just 7.2\% are validation (4.3\% evaluation and 2.9\% comparison).
%
Similarly, WildChat notes just 6.3\% of their LLM queries are factual QA \cite{zhao2024wildchat}.\footnote{It is not explicitly stated if these are even validation tasks, so this is another \textit{upper} bound of validation task prevalence.}
Thus, >90\% of queries are likely generative tasks (code, writing, or explanations), which MCQs struggle to test~(\cref{subsection:best_answer}).

% % \jbgcomment{I haven't checked this,
%   but if I remember it correctly, it is predictive, just less
%   predictive than other features.  This is still useful (if I'm
%   remembering correctly) for the story: grad admissions got rid of
%   multiple choice but kept the generative parts.}

Informative evaluation suites must reflect LLM use cases.
%
This is precisely why \mcqa exams are waning in graduate admissions
criteria: they cannot fully predict graduate school
success~\cite{sampson2001gre}. 
%
Similarly, over-representing \mcqa in evaluations obscures which LLMs best aid users.

\subsection{\mcqa Does Not Fully Test Knowledge} \label{subsection:testing_what}

While \mcqa fails to match user needs, we assume the format may test basic skills for such needs, justifying its usage.
%
\mcqa is meant to test knowledge \cite{moss2001multiple}, and with input texts, comprehension \cite{farr1990description}.
%
However, research in education reveals \mcqa may be suboptimal for these goals.

 MCQs mainly assess the basic knowledge levels in Bloom's Taxonomy of educational goals \cite{krathwohl2002revision}: recalling, understanding, and applying knowledge \cite{simkin2005multiple, shin-etal-2024-generation};
it is hard to write MCQs for the higher levels requiring reasoning \cite{stupans2006multiple, palmer2007assessment, lin2012can}: analyzing, evaluating, and creating knowledge.
As evidence, students can solve MCQs without full understanding, exposed in free-response answers \cite{mckenna2019multiple}.
%
MCQs with passages generally test comprehension, but some doubt this;
\citet{ozuru2013comparing} find \mcqa scores correlate with prior knowledge of the passage, overestimating true comprehension.

% In all, \mcqa may reliably test students' comprehension, but not full knowledge assessments.
We believe these same insights can apply to \abr{nlp}: \mcqa may be apt for
comprehension, but rewards LLMs for basic recall versus in-depth
knowledge.


==> 2025_acl_mcqa_sucks/pages/35_fix_format.tex <==
\input{figures/formats}

\section{\underline{Generative} \mcqa Tasks are Promising} \label{section:fixing_format}

\mcqa is flawed, so how should its role change?
Standardized LLM evaluations must 1) proxy LLM use cases; and 2) test skills for (1).
\mcqa is unfit for (1), so~evaluations need more tasks matching LLM needs (\cref{subsection:use_cases}).
Writing/explanation tasks are hard to score \cite{charney1984validity, chakrabarty-etal-2022-help, balepur-etal-2023-expository}, but it is still odd they are often omitted, as they are typical needs~(\cref{subsection:use_cases}).

This limits \mcqa to (2), but it is best for comprehension or validating objective facts (\cref{subsection:best_answer}), not generation, subjectivity, or knowledge (\cref{subsection:testing_what}).
Validation/comprehension are valuable, which is why we discuss \mcqa datasets in \cref{section:dataset}, but we need~better formats for the other skills.
Thus, we give two generative versions of \mcqa to better test LLMs (Figure~\ref{fig:format}):
Constructed Response (\cref{subsection:constructed_response}), answering sans choices, and Explanation \mcqa (\cref{subsection:justified_mcqa}), justifying predictions.
We ensure the formats only slightly increase evaluation complexity, mostly preserving \mcqa's simplicity of scoring. 
We now~describe the formats and future work to realize them.

\subsection{Constructed Response Questions} \label{subsection:constructed_response}

Having LLMs solve MCQs without choices, called \textbf{Constructed Response (CR)} in education \cite{livingston2009constructed} or short-form QA in \abr{nlp} \cite{krishna-etal-2021-hurdles}, is one better format.
CRQs test answer \textit{generation} unlike MCQs (\cref{subsection:best_answer}), better mirroring LLM needs (\cref{subsection:use_cases}), and it is easier to write CRQs testing all skills in Bloom's Taxonomy \cite{krathwohl2002revision}, so they better expose knowledge gaps (\cref{subsection:testing_what}).
Thus, students find CRQs harder than MCQs~\cite{hancock1994cognitive}, which can also delay saturation (\cref{subsection:saturation}).

Instead of writing CRQs to replace our vast existing \mcqa data, a promising solution is to convert MCQs into CRQs by omitting choices and tasking LLMs to give a \textbf{short-form} answer $\hat{a}$ for question $q$, comparing it to gold answer $a \in \mathcal{C}$ \cite{bhakthavatsalam2021think}.
\citet{myrzakhan2024open}~show two hurdles in this: finding MCQs to convert\footnote{\;``Which of these best...'' MCQs require using all choices.} and scoring $\hat{a}$ with $a$. 
Recent efforts in flagging MCQ errors \cite{moore2023assessing, moore2024automatic} and judging short-form answer correctness \cite{li-etal-2024-pedants, moore2022assessing} showcase that we can realistically overcome these challenges.
Thus, we~believe~combining this work with best practices for creating~CRQs \cite{snow2012construct} can successfully implement the task.

% Reliable MCQ to CRQ conversion would thus require combining advancements in MCQ generation \cite{lee2024math} and automatic scoring \cite{li-etal-2024-pedants} with best practices for writing and evaluating CRQs~\cite{snow2012construct}.

\subsection{Explanation Multiple Choice Questions} \label{subsection:justified_mcqa}

Constructed Response is promising (\cref{subsection:constructed_response}), but using one short answer is unfit for subjectivity \cite{lin2020differentiable} and conflicts user preferences for long outputs \cite{zheng2024judging}.
We thus propose~\textbf{Explanation \mcqa (\emcqa)} as another \mcqa alternative from education \cite{lau2011guessing}: for a question $q$ and choices $\mathcal{C}$, models give an answer $\hat{a} \in \mathcal{C}$ and explanation $\mathcal{E}$ for why $\hat{a}$ is right.
This format tests generation (\cref{subsection:best_answer}), matches the use case of explanations (\cref{subsection:use_cases}), and has shown to test more knowledge levels over \mcqa \cite{lee2011validating}.

%This format is also supported by education research, as asking for justifications can expose student knowledge gaps and heighten task difficulty \cite{tamir1990justifying, koretsky2016written}.

We envision \emcqa being treated like reasoning tasks \cite{cobbe2021training}, checking if LLMs pick $a$ like \mcqa's simple scoring, but also studying $\mathcal{E}$.
If models select $a$ but justify it poorly, it exposes knowledge gaps like in student assessments \cite{jonassen2010arguing}, and when models give strong explanations for wrong answers, it enables partial credit for subjective tasks \cite{lau2011guessing}.

\emcqa has many benefits, but needs metrics to score ``good'' explanations over many facets \cite{xu2023critical}, like factuality to curb hallucinations \cite{min2023factscore, balepur-etal-2023-text}, plausibility for convincingness \cite{liu2023vera}, and faithfulness to verify $\mathcal{E}$ supports $a$ \cite{lanham2023measuring}.
We believe these goals could be achieved by merging ongoing efforts in building verifiers for LLM reasoning \cite{NEURIPS2023_72393bd4} with educational best practices for grading justifications \cite{jonassen2010arguing}, yielding reliable metrics that realize \emcqa's potential.
\citet{kim-etal-2025-biggen} have made notable progress for this goal---building LLM judges to score justifications across various benchmarks---showing that implementing E-MCQA is feasible.


% \subsection{So... How Should I Evaluate My LLM?} \label{subsection:choosing_task_formats}

% As we have flagged many issues with \mcqa, \textit{how should we evaluate our LLMs?}
% For specific use cases, the ideal approach is to curate tasks that closely mirror deployment settings \cite{saxon2024benchmarks}.
% However, we often need general-purpose evaluations, tradeoffs arise between alignment with real-world use cases and evaluation cost and scalability. Human or LLM-based ratings align closely with downstream tasks but are costly and subjective. In contrast, \mcqa offers efficient and objective scoring but sacrifices generative alignment and real-world applicability. Our proposed alternatives, Constructed Response Questions and Justified \mcqa, offer a middle ground: they retain \mcqa’s simplicity and scalability while better reflecting LLMs’ generative capabilities. These formats could serve as practical, scalable solutions for evaluating general model capabilities and bridging gaps in existing benchmarks.

% We also don't mean to use our proposed formats to eliminate \mcqa.
% The ability of models to discriminate and pick high-quality answers via \mcqa formats is still valid and worth testing, especially as LLMs become more practically used for things like LLM-as-a-judge and (something else).
% This is why, in the next section, we discuss ways to improve current \mcqa datasets, which can also improve our alternative task formats that rely on \mcqa data. Everyone wins





% Testing how LLM calibration in MCQA impacts human confidence \cite{steyvers2024calibration}

% Conformal prediction to assess confidence \cite{kumar2023conformal}

% Answer-level calibration improves MCQA reliability and finds some data biases \cite{kumar2022answer}

% Uncertainty datasets/benchmark \cite{raina-gales-2022-answer, wang2024ubench}

% Prompt engineering can improve calibration \cite{ma2023prompt}


==> 2025_acl_mcqa_sucks/pages/40_dataset.tex <==
\section{\mcqa Datasets are Flawed but Fixable} \label{section:dataset}

\mcqa is not always the best format (\cref{section:format}), but we still need high-quality MCQs for comprehension/validation, along with tasks like LLM-as-a-judge \cite{gu2024olmes} and re-ranking \cite{ma-etal-2023-large} which require comparing answers.
Also, our generative \mcqa formats (\cref{section:fixing_format}) still use MCQs as inputs.

However, like most \abr{nlp} tasks, \mcqa datasets have quality issues that impede their utility: leakage
(\cref{subsection:test_set_leakage}), unanswerability
(\cref{subsection:quality}), shortcuts (\cref{subsection:artifacts}),
and saturation (\cref{subsection:saturation}).
We now show how educators' solutions to these issues can inform \abr{nlp} datasets.



\input{pages/41_leakage}


\input{pages/42_unanswerable}

\input{pages/43_shortcuts}

\input{pages/44_saturation}


==> 2025_acl_mcqa_sucks/pages/41_leakage.tex <==

% \jbgcomment{I think it's better for filenames to be named so that they sort correctly}

\subsection{LLMs Peek at \mcqa Answer Keys} \label{subsection:test_set_leakage}

To build an \mcqa dataset, we first need sources to write or collect
MCQs.
%
But as many sources end up being leaked\footnote{gpt-3 has seen
45\% of RACE's test set \cite{sainz2023nlp}.} in LLM training data
\cite{magar2022data}, such MCQs may confuse~generalization abilities for
memorization \cite{lewis2020question}.
%
Private test sets \cite{sap2019socialiqa} and de-contamination
\cite{zhou2023don} help, but LLMs tuned on newer data can overlap with
(1), and opacity in LLM data \cite{soldaini2024dolma} blocks (2).
% \jbgcomment{Patrick Lewis's paper on NQ overlap is probably worth citing here}

An ambitious solution to test set leakage is live MCQs that update over time to stay unseen \cite{white2024livebench}, like how educators rewrite exams to limit cheating.
In fact, trivia \cite{jennings2007brainiac}~and standardized testing groups often write new questions, making them ideal partners.
To aid both~parties, researchers could offer these groups tools for tutoring \cite{li-etal-2024-eden}, MCQ validation \cite{yu-etal-2024-automating-true}, or answer scoring \cite{yang-etal-2020-enhancing}.

Test set leakage would be easier to fix if model designers released
training data, but as we all know, most do not.
%
While it is harder to aid these efforts with methods that do not require training data, we hope researchers view it as
a challenging, impactful research problem in evaluation and
generalization.


==> 2025_acl_mcqa_sucks/pages/42_unanswerable.tex <==
\subsection{Some MCQs Have No Correct Answer} \label{subsection:quality}

Once a source is found (\cref{subsection:test_set_leakage}), researchers collect~or write MCQs, but errors often arise rendering them unanswerable, like mislabeling \cite{explained2023smart}, multiple correct choices \cite{Palta2024PlausiblyPQ}, ambiguity \cite{gema2024we}, missing contexts \cite{wang2024mmlu}, and grammar errors \cite{chen2023hellaswag}.

Educators write MCQs with rigorous protocols, and we must meet similar standards in \abr{nlp} \cite{boyd2019question}; we should use educators' rubrics (Figure~\ref{fig:checklist}) for writing and validating MCQs \cite{haladyna1989taxonomy}.
Such guidelines also specifically exist for distractors \cite{haladyna2002review}---the part of MCQs that discern testees' skills---ensuring they are truly wrong, shortcut-proof (\cref{subsection:artifacts}), and not too easy to rule out (\cref{subsection:saturation}).
Beyond MCQ writing, rubrics can form~data cards \cite{pushkarna2022data} to help researchers record errors in their data and how~they~fixed them.

Recent work in LLM checklist evaluation \cite{cook2024ticking}, 
MCQ metrics \cite{moon2022evaluating},~and MCQ generation \cite{feng-etal-2024-exploring} show parts~of this may be
automatable (Figure~\ref{fig:checklist}).
For instance, \citet{wang2024mmlu} fix errors in MMLU by using LLMs to detect issues and
write new choices.~LLM judges are not always reliable \cite{xu-etal-2024-pride}, so
human-\abr{ai} collaboration, like model-assisted
refinement~\cite{shankar2024validates} and task
routing~\cite{miranda2024hybrid}, may be more promising.
%
Errors will arise in MCQ writing, but educators' rubrics can help
find and fix them, ensuring answerability.

\input{figures/checklist}

==> 2025_acl_mcqa_sucks/pages/43_shortcuts.tex <==
\subsection{\mcqa Shortcuts May Let LLMs ``Cheat''} \label{subsection:artifacts}

Answerable MCQs (\cref{subsection:quality}) are not always high quality, as shortcuts may let LLMs guess the answers to MCQs without knowing the answers \cite{10.1145/3596490}, overestimating model accuracy \cite{wiegreffe2021teach}.
%
Shortcuts can arise from annotator artifacts \cite{gururangan2018annotation}, spurious patterns \cite{zhou2023explore}, or bypassed reasoning steps \cite{chen2019understanding}.
%
If LLMs best random guessing via partial inputs (e.g. choices only) \cite{richardson2020does}, they may~exist.

Below, we discuss how scoring (\cref{subsubsection:shortcut_scoring})
and data collection methods (\cref{subsubsection:shortcut_dataset})
can mitigate shortcuts.

% \jbgcomment{Note for the future: if YooYeon's AdvCal paper gets in, that should be cited here (or in RW) as well}

\subsubsection{Calibrated Scoring Can Deter Guessing} \label{subsubsection:shortcut_scoring}

While rare in human testing,\footnote{Since
they may induce stress or anxiety in students~\cite{vanderoost2018elimination},
but we think it is fine to stress~LLMs.} scoring methods can
penalize wrong guesses~\cite{lau2011guessing}:
\textbf{1) Probability scoring:} elicit confidence scores for each choice \cite{finetti1965methods}; \textbf{2) Negative marking:} subtract points for wrong answers with abstention allowed \cite{holt2006analysis}; and \textbf{3) Elimination scoring:} students iteratively remove wrong choices until unsure \cite{ben1997comparative}.
Confidence \cite{li-etal-2024-think}, abstention \cite{goral2024wait}, and elimination \cite{ma2023poe} have been studied in LLMs, so they may be easy to use for \mcqa evaluation.

These methods deter guessing, but also reward calibrated models that know their knowledge gaps \cite{guo2017calibration}.
While often ignored in evaluations \cite{bommasani2023holistic},
calibration scoring could let \mcqa better test decision-making \cite{liu2024dellma} and enable partial credit for subjective tasks where multiple choices may be tenable~(\cref{subsection:testing_what}).



\subsubsection{We Can Design Shortcut-Proof MCQs} \label{subsubsection:shortcut_dataset}

Data designers should limit shortcuts; an easy way is
uniform design.
When solving MCQs with only choices,
\citet{Balepur2024ArtifactsOA} find LLMs may exploit distributional
differences, so like educators~do (\cref{subsection:quality}), we should write parts of MCQs consistently: via the same agent, source, and decoding method.
%
HellaSwag \cite{zellers2019hellaswag} leads to the highest known choices-only accuracy, where \textit{user}-written answers and \textit{model}-written distractors are inconsistent, showing the necessity of uniform data design.

Contrast sets are another tool that detect if models ignore inputs and use shortcuts \cite{Gardner2020EvaluatingML}.
%
In \mcqa, they are entry pairs differing by some inputs (e.g. question)
that change the answer (Figure~\ref{fig:contrast}), ensuring models attend to the perturbed input
\cite{elazar2023measuring}.
%
\citet{balepur2024your} use contrast sets in commonsense \mcqa to
ensure none of their LLMs rely on shortcuts in choices to rank
highly.
%
Contrast sets are often made manually \cite{Kaushik2020Learning}, so future work~can test
automatic ways to build them \cite{li-etal-2020-linguistically}.

% \jbgcomment{self cites are a little prevalent here, pare back if you can}

% \cite{srikanth-rudinger-2022-partial}

Studying how users and models \textit{``cheat''}
\cite{saxon-etal-2023-peco} in MCQs also finds shortcuts.
%
In reading comprehension, \citet{Pang2021QuALITYQA} give~users \inlinecode{ctrl+F} to detect MCQs quickly solvable without using the full text, while \citet{Malaviya2022CascadingBI} flag MCQs where users
can use simple heuristics.
%
We can also train models to cheat; adversarial
filtering trains simple models
(e.g. bag-of-words) and omits MCQs they can solve \cite{zellers2018swag}.~Extending this, we believe having strong LLMs reason to cheat---similar to safety work in alignment faking
\cite{greenblatt2024alignment}---can help find shortcuts.


==> 2025_acl_mcqa_sucks/pages/44_saturation.tex <==
\subsection{LLMs Inevitably Ace \mcqa Datasets} \label{subsection:saturation}

Even if we fix all of these issues, MCQs become too easy over
time (i.e. saturated), no longer tracking LLM progress
\cite{li2024crowdsourced}.
%
To still use ``easy'' \mcqa datasets, we need to
make them harder for models.
%
% \jbgcomment{this sentence could be more direct: ``propose'' and ``study'' are filler words in academic writing}
Below, we show how understanding which MCQs
are hard (\cref{subsection:irt}) and helping users author hard, interpretable MCQs (\cref{subsection:hitl}) delay saturation.


\input{figures/contrast}

\subsubsection{IRT Reveals Challenging MCQs} \label{subsection:irt}

When LLMs excel in \mcqa datasets, some MCQs remain hard; finding
them and why they are hard informs data design
\cite{sugawara2018makes, Sugawara2022WhatMR}.
One MCQ difficulty metric is success rate (\success)---the number of models
answering correctly \cite{gupta2024improving}---but \success omits
\textit{which} models succeed.
MCQs solved by just the worst or best model have equally low success rates, but the former suggests MCQ errors (\cref{subsection:quality})---as a weaker model besting all others is rare---while the latter matches our expectation. 
As \success conflates these cases, it cannot separate flawed MCQs from those discerning model~ability.

% \jbgcomment{I think the better argument that IRT is better than SR is
%   that bad questions can have a low success rate: you want to
%   eliminate questions with errors, ambiguities, etc.  And leave the
%   discriminative questions.  You already introduced why you want
%   discriminative questions, so you can just back point to that.  I'd
%   talk more about the failure modes of SR, which can highlight how the
%   opposite of those are things IRT can find.}

Item Response Theory (IRT), a tool used in education \cite{lord2008statistical}, is a stronger way to find harder MCQs.
%
While success rate treats all models equally, IRT learns the skill of all models which then estimates each MCQ's difficulty (how hard it is) and discriminability (how well it discerns between weak/strong models).
IRT can then~filter high-difficulty and high-discriminability MCQs as harder subsets \cite{polo2024tinybenchmarks}, detect saturation if all MCQs have low difficulty and discriminability \cite{vania2021comparing}, and omit erroneous MCQs with negative discriminability \cite{rodriguez-etal-2021-evaluation}.

% rodriguez-etal-2021-evaluation

While IRT-based filtering finds harder MCQs, it does not give new MCQs, limiting its long-term use.
However, we can extend IRT to multi-dimensional IRT \cite[MIRT]{reckase200618} to capture \textit{many} latent skills, offering more insights into model abilities; by interpreting these skill dimensions, we can pinpoint model issues that inform future data efforts (\cref{subsection:hitl}).
\citet{gor2024great} reveal LLM errors in abductive reasoning via a variant of MIRT---an issue confirmed by abduction research \cite{del-fishel-2023-true, DBLP:conf/iclp/NguyenGTSS23}.
MIRT could similarly find difficult \mcqa topics, distractor patterns, or reasoning types for models \cite{benedetto-etal-2021-application}.

% \cite{balepur2024reverse}

% \jbgcomment{Density of self-cites a little high here (for the group, not just you)}

Overall, IRT can find which MCQs are hard but also why, informing future data collection efforts.

% \jbgcomment{Section title doesn't cover adversarial questions that well.  Perhaps a transition of the form: while engaged authors are used to understanding what trips up humans, they may need interface / computational support to trip up models\dots

% That could transition to adversarial data.}

\input{figures/adv}

\subsubsection{A Good MCQ is Hard \textit{and} Interpretable} \label{subsection:hitl}

A popular way to write harder MCQs is requiring obscure knowledge
(Figure~\ref{fig:adv}, left), sourcing from experts
\cite{rein2023gpqa, phan2025hle} and global competitions
\cite{fang2024mathodyssey}.
%
These challenge models \textit{and} humans, which is useful for \abr{ai} safety work in scalable oversight \cite{bowman2022measuring}.
However, this makes them uninterpretable for non-experts diagnosing model errors, especially when studying model rationales (\cref{subsection:explanations}).
If LLMs~err on obscure MCQs, it is hard for non-experts to find if errors are from faulty reasoning, misunderstandings, or knowledge gaps \cite{anderson2025phdknowledgerequiredreasoning}.

While authors know which MCQs elude humans, writing ones that surface model errors while staying human-interpretable needs support.
This is \textbf{adversarial} data collection's goal \cite{kiela-etal-2021-dynabench}---building UIs to help authors write examples hard for models but easy for humans (Figure~\ref{fig:adv}, right).
Rather than using niche knowledge, authors must write MCQs with spurious patterns, misleading distractors (\cref{subsection:quality}), or reasoning traps that trick LLMs but not humans \cite{xu2023llm}.
As a result, these MCQs better expose robustness (\cref{subsection:robustness}) and logical reasoning (\cref{subsection:explanations}) errors, less clouded by knowledge.

Adversarial MCQs are useful, but finding users to write high-quality ones is tough.
Gamification---making the task fun---helps, shown by successful adversarial commonsense \cite{talmor2022commonsenseqa}, QA \cite{wallace2019trick}, and fact-checking \cite{eisenschlos2021fool} datasets.
\citet{wallace-etal-2022-analyzing} use gamification to build adversarial NLI data and show it has \textit{long-term} difficulty, delaying saturation. 
% \citet{sung2024your} recently use gamification with IRT (\cref{subsection:irt}) to build an adversarial QA dataset with the highest gap in human and model accuracy in the past five years.
For even more engagement, researchers can stir users to author MCQs exposing shocking failure cases, inspired by jailbreaking, where provocative outputs are naturally fun to elicit \cite{schulhoff2023ignore}.
%\cite{schulhoff2023ignore}.

% \jbgcomment{DADC would be better for submission (the barrage of self-cites can return for camera ready, so don't delete, jsut comment)}

Obscure and adversarial MCQs can both make \mcqa harder: the former
tests niche knowledge, while the latter better finds reasoning or
consistency failures that are uneclipsed by knowledge gaps.


==> 2025_acl_mcqa_sucks/pages/50_models.tex <==
\input{figures/llm_issues}

\section{Fixing \mcqa Can Help Us Fix LLMs} \label{section:models}

Fixing issues in \mcqa's format (\cref{section:format}) and datasets (\cref{section:dataset}) will not just improve evaluation quality; they can also improve our understanding of LLM weaknesses.
This section outlines three persistent
issues of LLMs in \mcqa (Figure~\ref{fig:llm_issue})---robustness~(\cref{subsection:robustness}), bias
(\cref{subsection:bias}), and explanations
(\cref{subsection:explanations})---and how our prior solutions can better address or evaluate them.


\subsection{New Prompts Lead to New \mcqa Scores} \label{subsection:robustness}
% \subsection{LLMs Lack Robustness in \mcqa} \label{subsection:robustness}

% On specific prompts, LLMs score highly in~\mcqa, but currently crumble
% when prompts change, sensitive to: choice
% symbols~\cite{alzahrani2024benchmarks}, choice
% order~\cite{pezeshkpour2023large, Zheng2023LargeLM}, and
% phrasing~\cite{holtzman-etal-2021-surface, Wiegreffe2023IncreasingPM}.
% This brittleness weakens \mcqa leaderboard reproducibility, as varied
% setups yield conflicting rankings~\cite{gu2024olmes}

On specific prompts, LLMs score highly in~\mcqa, but currently crumble
when prompts change, sensitive to: choice
symbols \cite{alzahrani2024benchmarks}, choice
ordering \cite{Zheng2023LargeLM}, and
phrasing \cite{Wiegreffe2023IncreasingPM}.
This brittleness degrades \mcqa leaderboard reproducibility, as varied setups produce conflicting rankings~\cite{gu2024olmes}


LLM robustness varies by task setup.
%
In \mcqa, early LLMs with poor instruction
following \cite{zhang2022opt} used probability-based \textit{scoring},
while instruction-tuning enabled LLMs to \textit{generate}
answers \cite{longpre2023flan}; while logically equivalent, these give varying answers \cite{lyu2024beyond}. 
Probability scoring seems more at fault---more sensitive to prompts \cite{wang2024look}---doubting if LLMs can aid decision-making tasks that need accurate confidence scores \cite{liu2024dellma}.
To track this progress in LLMs, researchers can use \mcqa scoring protocols that measure calibration~(\cref{subsubsection:shortcut_scoring}).

As accuracy often \textit{drops} post-perturbation \cite{zhou-etal-2024-revisiting}, these failures in generalization could indicate dataset leakage (\cref{subsection:test_set_leakage}) or over-reliance on biases (discussed in \cref{subsection:bias}).
Another proposed explanation is symbol binding error: LLMs ``know'' the right answer but cannot link it to the correct choice \cite{Wiegreffe2024AnswerAA, xue2024strengthened}.
These failures weaken \mcqa's ability to test knowledge, obscured by memorization and symbol binding.\footnote{Such evaluations have downstream use (e.g. privacy, interpretability), but do not truly measure knowledge as intended.}~Our proposed solutions---like curating live MCQs for data leakage (\cref{subsection:test_set_leakage}) and generative \mcqa formats to expose knowledge gaps without needing symbol binding (\cref{section:fixing_format})---can more reliably assess knowledge.

% \jbgcomment{If short on space, some of these could be move to appendix}

\subsection{LLMs are Biased \mcqa Test-Takers} \label{subsection:bias}

Like most \abr{nlp} tasks \cite{baumler2022recognition, chu2024fairness}, LLMs exhibit biases in \mcqa, grouped into two main types.
%
% \jbgcomment{can we be a little more precise than ``favor''?}
%
The first are \mcqa-specific biases---selecting answers based on symbols \cite{Zheng2023LargeLM}, positions \cite{Li2024CanMQ,
wei-etal-2024-unveiling}, or phrases such as ``none of the
above'' \cite{xu2024llms, wang2025llms} rather than MCQ content.
This degrades robustness
(\cref{subsection:robustness}), masking model knowledge.
%
We believe they likely stem from shortcuts (\cref{subsection:artifacts});
%
LLMs tuned on data where choices with patterns are often
correct will exhibit these biases~\cite{pacchiardi2024leaving}.
%
Our safeguards---uniform design, contrast sets,
and ``cheating'' (\cref{subsubsection:shortcut_dataset})---can
reduce these biases, and more work in shortcuts may be key
to quash them.

The second bias type stems from general training, like cultural/linguistic bias \cite{myung2024blend, li2023land};
LLMs often err on non-Western cultural MCQs \cite{Acquaye2024SusuBO, azime2024proverbeval} and non-English MCQs \cite{son2024kmmlu, li2023cmmlu}.
MCQs are popular for testing bias \cite{guo2023evaluating}, but if they use subjective commonsense \cite{seo-etal-2024-kocommongen}, they are subpar (\cref{subsection:best_answer}).
Thus, we advise writing MCQs with rubrics to limit ambiguity and correct distractors (\cref{subsection:quality}),~ensuring bias is more objectively tested.
If subjectivity persists, evaluators should consider ways to handle it like our~proposed Explanation MCQA (\cref{subsection:justified_mcqa}) or calibration scoring (\cref{subsubsection:shortcut_scoring}), aiding bias testing and for \emcqa, better matching how bias presents downstream \cite{seshadri2025does}.

Lastly, to construct non-English MCQs, we note that researchers typically either: 1) collect MCQs in the desired target language \cite{son2024kmmlu}; or 2) translate English ones \cite{achiam2023gpt};
However, (1) may be infeasible for languages that are low-resource or where \mcqa is rarely used,\footnote{In Germany it is uncommon to test students with MCQs: https://www.reddit.com/r/AskAnAmerican/comments/rjxns4/} while (2) may introduce error propagation during translation \cite{singh2024global}---showing neither method is perfect on its own.
Thus, our prior solutions can be adopted to benefit both methods---like using rubrics during translation (\cref{subsection:quality}) or collecting non-English MCQs from unseen sources (\cref{subsection:test_set_leakage})---improving evaluations of multilingual abilities.

\subsection{LLMs Struggle to ``Explain Their Work''} \label{subsection:explanations}

% LLMs can easily pick MCQ answers~(\cref{subsection:saturation}), but often give \textbf{unfaithful} explanations---failing to mirror their true reasoning---whether via chain-of-thought \cite{lyu2023faithful, lanham2023measuring, turpin2024language} or self-explanations \cite{agarwal2024faithfulness, kim2024can, madsen2024self}.
% However, they are convincing, surpassing crowdworkers in perceived quality \cite{mishra-etal-2024-characterizing} and misleading humans when incorrect \cite{si2023large}, likely due to LLM alignment protocols that optimize user preferences instead of accuracy \cite{wen2024language}.

Even if LLMs get the right answer to an~MCQ, they may justify their selection \textbf{unfaithfully}---failing to mirror their true reasoning---whether via chain-of-thought \cite{lyu2023faithful, turpin2024language} or self-explanations \cite{kim2024can, madsen2024self}.
However, they are convincing, besting crowdworkers in judged quality \cite{mishra-etal-2024-characterizing} and misleading users when wrong \cite{si2023large}, likely as standard alignment strategies tend to optimize LLMs for user preferences over helpfulness \cite{balepur-etal-2024-smart, wen2024language}.

LLM explanation flaws are even clearer after logical consistency checks.
\citet{kawabata2023evaluating} show LLMs often inaccurately explain answers to subquestions in reading comprehension, even when answering the higher-level question correctly.
Similarly, \citet{balepur-etal-2024-easy} find LLMs struggle to reason why distractors are wrong.
These issues likely stem from broader LLM logical inconsistencies \cite{liu2024aligning, varshney2024investigating}.

Explanations are popular LLM use cases~(\cref{subsection:use_cases}), highlighting the need for improved \mcqa formats such as Explanation MCQA (\cref{subsection:justified_mcqa}) which explicitly test explanation skills.
Further, LLMs' logically inconsistent explanations offer a path toward harder datasets (\cref{subsection:saturation}); tools like MIRT (\cref{subsection:irt}) can identify logical error types (negation, decomposition) that elude LLMs, while adversarial collection can curate MCQs to excise these errors while staying easy for humans (\cref{subsection:hitl}).
In all, LLMs' poor explanation abilities give an opportunity to design harder \mcqa evaluations better aligned with user needs.




% \subsection{Shortcuts}

% Word level shortcuts in MCQA \cite{pacchiardi2024leaving}

% BERT can do MRC without the passage, random keywords distract BERT, perturbations change accuracy \cite{si2019does}

% More MRC shortcuts \cite{Yu2020CounterfactualVC}

% Quantifying the learnability of shortcuts \cite{Shinoda2022WhichSS}

% MRC doesnt need the input passage \cite{raina2023analyzing}

% MRC doesnt need the input passage, neither do humans \cite{liusie2022world} 

% Easy to cheat on MCQA versions of multi-hop datasets \cite{chen2019understanding}


% \subsection{Future Directions}

% Interpretability via contrastive edits \cite{ross2020explaining}

% Interp via circuits \cite{lieberum2023does}

% Interpreting biases \cite{shen2022understanding}

% AI Safety --- some MCQA tasks are hard for humans, we can study models in relation to helping humans \cite{parrish2022single, parrish2022two, wen2024language}


==> 2025_acl_mcqa_sucks/pages/80_limitation_ethics.tex <==
\section{Limitations} \label{section:limitations}

Inspired by \citet{saxon2024benchmarks}, we organize our limitations section as potential counterarguments:



\paragraph{I Do Not Work on \mcqa:}

Our approach to \mcqa can apply to all tasks;
it is important to question if your format effectively evaluates your intended ability.
Educators have long-studied the best formats for different tasks, but we are not using these insights to guide our benchmark design.
As an example beyond \mcqa, in human math assessments, students are often required to ``show their work'' to verify understanding and diagnose misconceptions \cite{choy2016snapshots}. However, math datasets like GSM8k \cite{cobbe2021training} often ignore intermediate computations in their metrics.
Similarly, our dataset quality issues are universal; it is always important to ensure datasets are not contaminated or saturated, as well as free from errors and shortcuts.
Thus, we advise all researchers---regardless of task or domain---to consult education research to see if they can improve their evaluations' efficacy.

\paragraph{Other modalities, languages, etc. are different:}
Our critiques of \mcqa's rigid goals (\cref{subsection:best_answer}), misalignment with user needs (\cref{subsection:use_cases}), and failure to fully assess knowledge (\cref{subsection:testing_what}), along with our proposed generative task alternatives (\cref{section:fixing_format}), are applicable regardless of modality and language.
Further, the \mcqa dataset quality concerns (\cref{section:dataset}) we discuss are still relevant to these domains;
for example, in some multi-modal QA datasets, models can answer questions without using the given input image \cite{goyal2017making}, showing shortcuts exist (\cref{subsection:artifacts}).

\paragraph{Why not abandon \mcqa?}

Indeed, other formats have grown in popularity, such as prompting LLMs on real-world user queries and using annotators or models to judge model responses \cite{chiang2024chatbot, lin2024wildbench}.
These efforts are exciting and can directly proxy LLM use cases, but are difficult to scale for every domain we currently use \mcqa for, their subjective scoring lacks reproducibility, and these metrics are easy to game \cite{zheng2025cheating}.
In contrast, \mcqa and our proposed generative formats include scoring using ``pick the best answer'', forming a more efficient and objective metric.
Thus, we should aim to advance both of these threads for more reliable evaluations.

\paragraph{This is All Way Too Much Work:}

We have proposed many directions for future research, but our objective is not to have every \mcqa dataset designer engage with each of these efforts.
We hope that by pointing out these issues in \mcqa, dataset designers will start to consider how using \mcqa will affect their datasets' reliability in the long term, and researchers will further study ways to improve \mcqa evaluation.
Even adopting just one of our proposals could greatly enhance the quality and effectiveness of \mcqa datasets.
Over time, these small, incremental improvements across the evaluation community will drive meaningful progress.

\paragraph{Generation is too Hard:}

While generative versions of MCQA are harder to implement, such efforts are warranted to improve the utility of evaluations: generation tasks better test knowledge (\cref{subsection:testing_what}) and mirror LLM use cases (\cref{subsection:use_cases}). We believe the difficulty of implementation should not preclude the adoption or at least exploration of these threads.

We agree MCQA is attractive as it is easy, but this is not the most important property of evaluations; evaluations should measure how the system will behave in deployment \cite{saxon2024benchmarks}.
LLMs are used to generate text that helps users, so we argue researchers should strive for tasks that measure generation, not just those that are easy to implement.
Many fields have also faced difficulty when evaluating their newest systems, like Information Retrieval and Machine Translation, and have thus made progress as a community toward new evaluation datasets \cite[e.g. TREC]{voorhees2001trec},  and metrics \cite[e.g. COMET]{rei-etal-2020-comet}; we should thus do the same for LLMs with MCQA.

Our proposed shift from validation to generation evaluations is also not totally new.
NLP saw a similar trend in summarization, where efforts switched from evaluating if systems could extract sentences within an input text to generating abstractive summaries \cite{mehta2016extractive}.
Abstractive summarization is harder to evaluate, but we made this change as a community as it better captured the downstream summarization needs of users \cite{lin2019abstractive}.

% \paragraph{Where are the Experiments?}



\section{Ethical Considerations}

Flawed evaluations can mislead both researchers and users; researchers may misinterpret model abilities due to quality issues in datasets, while users may struggle to identify the best models for their needs.
This paper outlines several potential solutions to mitigate these risks in \mcqa, ensuring more reliable evaluations for researchers and users.

%Overall, our findings provide broader insights to improve general evaluation practices beyond text-only \mcqa.

\section*{Acknowledgments}

We would like to thank the \abr{clip} lab at the University of Maryland and our external collaborators for their help.
In particular, we thank Paiheng Xu, Dang Nguyen, Shi Feng, Ioana Baldini, Vipul Gupta, and the Google Translate Reading Group for general discussions; Yu Hou, Dayeon Ki, and Connor Baumler for discussions of culture/biases; Maharshi Gor for feedback on IRT; Yoo Yeon Sung for feedback on IRT and adversarial data collection; Matthew Shu for feedback on best practices in educational testing; Atrey Desai for helping us test MCQ checklist evaluation; and Naina Balepur for brainstorming our excellent title.
We also appreciate Michael Saxon, Yi Ting Huang, Fumeng Yang, and Andrew Lan for reviews on earlier versions of this paper.
This material is based upon work supported by the National Science Foundation under Grant No. \abr{iis}-2403436 (Boyd-Graber), \abr{iis}-2339746 (Rudinger), and \abr{dge}-2236417 (Balepur).
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.

% Hope, Zoey, Connor (Bias)
% Maharshi (IRT)
% YY (Adversarial, IRT)
% Maharshi (IRT)
% Naina (Title)
% Matthew (Education)
% Michael (full review)
% Andrew Lam
% Yi Ting

==> scripts/style-check/bad-words <==
utilize              % phrase "use" http://www.bartleby.com/64/C003/0294.html
utilizes             % phrase "uses" http://www.bartleby.com/64/C003/0294.html
utilized             % phrase "used" http://www.bartleby.com/64/C003/0294.html
utilizing            % phrase "using" http://www.bartleby.com/64/C003/0294.html
leverage             % phrase "use"
abstraction          % phrase this is often used poorly?
fashion              % phrase hrm.
[dw]on't             % spelling do not or will not.
behavioral           % spelling I'm convinced we don't use this word properly.
we'll                % spelling we will
we've                % spelling we have
[^r][^c][^h] impact  % phrase "consequences", "effect", "result", though nsf likes "research impact"
tackle               % phrase "tackle" (a problem) is wimpy for "solve" or a tired metaphor for "address a challenge".
thusly               % phrase "thus" or "this way" or "like this" http://www.bartleby.com/64/C003/0282.html
transpire            % phrase "happen" 
so-called            % phrase can be abused; it's negative.
necessitate          % phrase require.
necessitated         % phrase required.
necessitates         % phrase requires.
loosing              % spelling you almost certainly mean "losing".  use "loosening" otherwise.
aforementioned       % phrase too pretentious.
important to         % phrase "valued by"?
notion               % phrase avoid this weak phrase. (thanks brian bershad!)
achieve(s)?\s        % phrase models don't achieve anything, only use for humans
reasonably           % phrase hedging


==> scripts/style-check/common-typos <==
a the                % phrase double article
 pt                  % syntax ? I guess avoid straggling pt's that escape tex?
[ ],                 % syntax whitespace before comma seems wrong.
Figure Figure        % phrase pizza pizza.
[ ]-[ ]              % syntax a hyphen surrounded by space should probably be an emdash '---'
[0-9]-[0-9]          % syntax use an endash '--' for ranges
[0-9]ms              % syntax put a space between the number and the unit.
[^egs]\. [a-z]       % syntax a period usually ends a sentence, and sentences should start with a capital; doesn't apply for i.e.,
\.  [a-z]            % syntax a period usually ends a sentence, and sentences should start with a capital; "i.e." should have a comma following.
[a-z]\.\.            % syntax double period is rarely right, use \ldots for ellipsis
[^\\]"               % syntax use fancy quotes
\beg\.               % syntax should be e.g. as in "examples given"
from to\b            % phrase haven't used this properly.
help help            % phrase double word, that probably means the author paniced
of of                % phrase apparent double word.
the affect           % phrase should probably be 'the effect'
the the              % phrase apparent double word.
there too few        % phrase there are too few?
was not was          % phrase pretty much a joke if this gets matched.
we we                % phrase it would be oi oi in french, I guess.
with on              % phrase probably wrong.
with with            % phrase apparent double word.
[\n ]--[\n ]         % syntax that's an en-dash, you want an em-dash: "---"
my my                % phrase unlikely that's what you want, at least without a comma. (doesn't work across newlines)
>From                % syntax be careful when you email .tex files.  I've seen this slip through into submissions.
e\.t\.c\.            % syntax it's et cetera; use etc.
such as like         % phrase pick one
<<<<<<< .            % syntax CVS conflict!
=======              % syntax CVS conflict!
>>>>>>> [0-9]        % syntax CVS conflict!
e\.g\.[\n ]          % syntax should be followed with a comma, as e.g. can be read as "for example" (thanks JZ!)
i\.e\.[\n ]          % syntax should be followed with a comma, as i.e. can be read as "that is" (thanks JZ!)
[ ]\.[\n ]           % syntax stray period?
further more         % phrase one word: furthermore
safe guard           % phrase one word: safeguard
that be              % phrase mistake.
can not              % phrase cannot
only only            % phrase double word
is is                % phrase double word.
they shows           % phrase argh, mistake.
less that than       % phrase typo damage
from from            % phrase double word score
in in                % phrase "in" (common mistake)
not not              % phrase argh.
it it                % phrase argh.
to illicit           % phrase "to elicit" -- illicit is always an adjective.
c\.f\.               % phrase actually, it's cf., and you'd like cf.\ (backslash space)
this lead to         % phrase "led to" if past tense, "leads to" if present.
on on                % phrase double word.
has is               % phrase choose
description their    % phrase saw this, clearly wrong.
including:  % syntax I prefer no colon after including, which already says a list is coming.
[a-z]\([A-Z]  % syntax put a space before parens, even when introducing acronyms.
without and without % phrase saw this.
can be result       % phrase saw this typo.



==> scripts/style-check/foolish-phrases <==
(quite|more|very|most) unique    % phrase unique is.
(quite|more|very|most) abstract  % phrase abstract is.
tangible view                    % phrase mix that metaphor some more.
for e\.g\.                       % phrase e.g. includes "for".
begs the question                % phrase unless you're very clever: "raises the question": http://alt-usage-english.org/excerpts/fxbegthe.html
high rate of speed               % phrase local news-speak.
especially necessary             % phrase 'especially important', necessary may be an absolute like unique.
how will it effect % phrase you likely meant "affect"
how it will effect % phrase you likely meant "affect"
insure proper performance % phrase "ensure"
especially true                  % phrase 'especially important', true may be an absolute like unique.
to affect change                 % phrase "effect" change;  I read this on a poster.
higher results                   % phrase maybe higher performance or higher values.
is more general then the         % phrase probably "than"
upper bounding                   % phrase "limiting" or "setting an upper bound on"
in principal                     % phrase likely, "in principle"
literally like                   % phrase literally means no simile.  
design principal  % phrase likely, "design principle" 
different from 	    	   	 % phrase unlike

==> scripts/style-check/latex-checking <==
\{\\em [^\}]*[^\}\/]\}[:]    % syntax use \emph{} or explicit italic correction {\em foo\/}
\{\\em [^\}]*[:\.,]\}        % syntax punctuation at the edges of italic text is not italicized
[A-Z]{2,10}\.[ ]*[\n ][ ]*[A-Z]  % syntax intersentence spacing should be used if a sentence ends with an acronym: "FOO\\@."
\\etal[^{]                   % syntax it's good practice to use \etal{} to avoid bad spacing
\\caption\[[^\]]*[^\.]\]     % syntax short caption should end with a period.
\\caption\[.*CCDF.*\]        % syntax short caption should not include graph type.
\\caption\[.*CDF.*\]         % syntax short caption should not include graph type.
\\caption\[.{0,25}\]         % syntax short caption should not be too short.
th century                   % syntax use textsuperscript
[ ]---[ ]                    % syntax the em-dash should be right up against the words.
[ \n]---[ \n]                % syntax the em-dash should be right up against the words.
^---[ \n]                    % syntax the em-dash should be right up against the words.
[ \n]---$                    % syntax the em-dash should be right up against the words.
[ \n]--[ \n]                 % syntax the en-dash should be between numbers.
^--[ \n]                     % syntax the en-dash should be between numbers.
[ \n]--$                     % syntax the en-dash should be rbetween numbers.
,[~ ]\\etal                  % syntax no comma before etal (unless Smith, Martinez, \etal)
\\etal\{\}'s                 % syntax eew.
\\(sub)?section\{[A-Z][^}]*[ ][a-z]{5,40}[^}]*\} % syntax subsection headers should be initial capped.
\\(sub)?section\{[A-Z][^}]*[^:][ ]{1,}(With|A|An|Is|And|For|To|The)[ ][^}]*\} % syntax some words needn't be capitalized
[ ]\\footnote                % syntax no space before footnote.
\\footnote\{.*\}.            % syntax footnotes after punctuation
,,                           % syntax double comma is unlikely to be intentional.
cf\.[^\\]                    % phrase cf. should get an escaped space "\ "
et al\.[^\\]                    % phrase et al. should get an escaped space "\ "
[<>]  % syntax a less than or greater than outside math mode shows other characters.
in (section|table|figure) \\ref % phrase should have ~ before ref
section~\\ref % capitalize capitalize section when saying Section 6.
table~\\ref % capitalize capitalize section when saying Table 6.
figure~\\ref % capitalize capitalize section when saying Figure 6.
\\(sub)?section\{Intro\} % syntax spell it out.
,''                          % syntax punctuation outside quotes
\.\.\.                       % syntax use \dots

==> scripts/style-check/my-rules <==
#  such may be abused to blacklist certain words even spelled correctly.
# capitalize is case sensitive, and also bracketed by non-word.
# phrase and spelling are case insensitive, but bracketed by non-word characters.
# syntax is case sensitive but not bracketed by non-word; probably best if used with regexes.
\bet al\.[^}]        % syntax use the \etal{} command instead. (or write one to italicize)
\bet\. al\.          % syntax use the \etal{} command, "et" needs no dot (et alii). (or write one to italicize)
\bc\.f\.\b             % syntax should be cf. for "confer" (latin for compare)
\b$i\)[^$]              % syntax leave the paren in math mode -- should be $i)$
\b$ii\)[^$]             % syntax leave the paren in math mode -- should be $ii)$
\b$iii\)[^$]            % syntax leave the paren in math mode -- should be $iii)$
\b$iv\)[^$]             % syntax leave the paren in math mode -- should be $iv)$
\b$v\)[^$]              % syntax leave the paren in math mode -- should be $v)$
\ban [b-df-gj-np-tv-z] % syntax probably meant to use "a" instead of "an", though there are exceptions.
\ban [B-DF-GJ-NP-TV-Z][^A-Z/] % syntax probably meant to use "a" instead of "an", though there are exceptions (like acronyms).
\b[Aa] [aeiouAEIOU](?!se|ni|A|ur|RL|ti|ne|DP) % syntax probably meant to use "an" instead of "a", though there are exceptions. (user, useful, AA, unified, uniform, unique, Europe, one, UDP; n/a doesn't work, so use {n/a})
This allows           % phrase tie more explicitly: This (x) allows...
we find               % phrase omit "we find"
we found              % phrase omit "we found"
try and               % phrase "try to", though if you're using try as a noun in a compound sentence, this rule is wrong.
impact of             % phrase not a useful metaphor; try evaluation, success, effect, value.
including [^\.]*etc\. % syntax "including" tells of a non-exclusive list, so "etc." is redundant.  This rule will misfire if you have two lists in your sentence, but you shouldn't do that either. ;)
includes [^\.]*etc\.  % syntax "includes" tells of a non-exclusive list, so "etc." is redundant.  This rule will misfire if you have two lists in your sentence, but you shouldn't do that either. ;)
and etc\.             % phrase come on. learn some latin.
AT&T                  % syntax you poor thing, this won't compile.
doesn't               % phrase be formal.
be occur              % phrase what happens when I'm indecisive about what follows "can"
up until              % phrase "until"
one or more           % phrase probably redundant -- nonzero is probably implied.
is comprise(d|s) of   % phrase you probably mean "is composed of" because "comprises" is more a synonym for "contains" 
will be significantly different % phrase "will differ significantly" for active voice
More importantly,     % phrase probably means the order is wrong: put important stuff first.
todo                  % ignoredcommand
texttt                  % ignoredcommand
jbgcomment              % ignoredcommand
lkfcomment              % ignoredcommand
due to space constraints % phrase don't whine.
this paper % phrase can be ambiguous if talking about someone else's paper whether you mean the one youre writing or the one you're talking about..
the above             % phrase horrible phrase that must be expunged.  you might use "these" instead, but best to make the sentence stand alone.
referred to above     % phrase "these".
(all|the|of) [0-9][ ] %  phrase use words for numbers in phrases.
clearly shows         % phrase "clearly" is usually much.
grows larger          % phrase is "grows smaller" possible?  grows.
guarantee as much as possible % phrase then not really a guarantee "provide"
affects negatively   % phrase "hurts" or "harms"
rely upon % phrase rely on is good enough
relies upon % phrase relies on is good enough
record route packets? % phrase hyphenate record-route packets
record-route; % phrase leave record route alone if not modifying something else
we accomplish this  % phrase verbose way to get active voice.
refers to the % phrase you're being wimpy in the definition.  use "is"
\\emph\{[a-zA-Z ]*\} refers to % syntax you're being wimpy in the definition.
loss off % phrase loss of?
this could % phrase this "what" could
with that has % phrase probably just one
simply % phrase probably isn't.
to get to % phrase "to reach"?
latency benefit % phrase reduction
latency improvement % phrase reduction
shed insight % phrase 'shed light' would seem the metaphor.
increasingly more % phrase redundant
I\.e\. % syntax starting a sentence with i.e. is just ugly.
E\.g\. % syntax starting a sentence with e.g. is just ugly.
in the large % phrase if large is a noun, bad.  if it's an adjective, fine.
encapsulates with % phrase seen it, don't know what it means.
when working with % phrase just say "with"
it is true that	  % phrase usually can delete
LDA % phrase convention put in small caps
(F|f)indings (show|indicate|suggest)	% phrase delete or make more specific

==> scripts/style-check/networking-research <==
IPs                  % phrase should be IP addresses
[Rr]ate-limits       % spelling "rate limits" has no hyphen, only "rate-limited"
best effort          % phrase hyphenate best-effort service.
deliver route        % phrase jargon redundancy
euclidean % capitalize Euclidean.
interdomain          % spelling inter-domain
internet             % capitalize unless talking about an internet other than the Internet
intradomain          % spelling intra-domain
log-normal           % spelling lognormal is one word.
pareto               % capitalize
ttl                  % capitalize
weibull              % capitalize proper name.
PoP                  % syntax I think POP looks less annoying.
PoPs                 % syntax I think POP looks less annoying.
http[ ]              % capitalize capitalize HTTP.
linux                % capitalize capitalize Linux
Internet[^\.]*Internet % syntax avoid Internet twice in the same sentence?
zipf                 % capitalize capitalize the guy's name.


==> scripts/style-check/nlp <==
Internet[^\.]*Internet % syntax avoid Internet twice in the same sentence?
[A-Z]{2,}[s]?[\.,\s]% capitalize Use small caps for acronyms

==> scripts/style-check/passive-voice <==
it is possible to                   % phrase passive voice, try: "can"
are identified by                   % phrase passive
is shown                            % phrase passive.
is not included in                  % phrase maybe this is passive
there (are|is) [^\.:;]* (that|in)   % phrase maybe this is passive
can be evaluated                    % phrase avoid passive: I evaluated
can be observed                     % phrase avoid passive: are visible
# is needed                         % phrase passive voice
is used to                          % phrase go active voice, or subsititute "helps"
(are|were) needed[^\?]              % phrase passive voice
(is|are) presented in               % phrase "appears in", or reword to avoid passive voice
it is possible that                 % phrase "may"
(is|are) (depicted|illustrated|sketched) in  % phrase thats passive voice
(is|are) shown in                   % phrase "shows"
as can be seen in                   % phrase X shows that Y.
there needs to be                   % phrase passive voice in a bad way.
was designed                        % phrase passive voce.
it may be                           % phrase passive "it"
it is important that                % phrase passive; replace with X is important because Y.


==> scripts/style-check/verbose-phrases <==
a large number of                   % phrase you mean "many"
a substantial number of             % phrase how substantial?  most?  or just enough that can't be ignored?
an insufficient number of           % phrase "too few"
a significant number of             % phrase one is significant.   consider "prohibitive" if the number is sufficient to be problematic.
a number of                         % phrase getting the verb agreement for this useless phrase is tricky.
a number of different               % phrase use "different" (should have a high score)
a small number of                   % phrase you mean "few"
a low number of                   % phrase you mean "few"
a relatively low number of                   % phrase you mean "few"
actually                            % spelling probably doesn't add
to an extent                        % phrase you can probably remove
and instead                         % phrase replace with but?
be done                             % phrase if "X of Y can be done", try "Y can be Xed"; it's already passive voice.
combining multiple                  % phrase as opposed to "combining one?"
aggregating multiple                % phrase "aggregating"
do this                             % phrase probably verbose if you use a pronoun for what you're doing
exists[ ]                           % phrase probably no better than "is", but end of sentence may be unavoidable?
if it is to                         % phrase should be "to" (usually followed by "be X")
if they are to                      % phrase should be "to" (usually followed by "be X")
in general                          % phrase unless matched with "in specific," this is usually useless; perhaps "overall"
in order to                         % phrase remove "in order" and get "to"
in the past                         % phrase past tense is likely enough.
in the way of                       % phrase should be "as"
counting the number of              % phrase counting.  dude.
is permitted to                     % phrase "may"
largely opaque                      % phrase largely does not modify opaque
makes a new                         % phrase should be "creates"
may not chose                       % phrase "may not" is future tense; "chose" is past.
one should note                     % phrase just write it.
note that                           % phrase is the rest of the paper less notable?
Note, that                          % syntax not only should you not "note that", no comma after note.
we note                             % phrase is the rest of the paper less notable?
note however that                   % phrase is the rest of the paper less notable?
it is important to note             % phrase is the rest of the paper less notable?
really                              % phrase probably doesn't add; if you think it does, use "r{}eally" -- don't change to 'in fact'
in fact				    % phrase cut
rigorously                          % spelling probably doesn't add, and I rarely do anything with rigor
the way in which                    % phrase should be "how" or ""
the manner in which                 % phrase should be "how" or ""
value stems                         % phrase value is derived or offered, I think.
time at which                       % phrase very likely "when"
place at which                      % phrase very likely "where"
at the time                         % phrase very likely "when"
reduced number of                   % phrase very likely "fewer" or maybe maybe "less"
is present in                       % phrase present is probably redudant, try "is in"
they all                            % phrase maybe "all xs" would be better.
easy to do                          % phrase "feasible" or "practical" might be better.
is going to                         % phrase "will".
are going to                        % phrase "will".
getting                             % phrase probably "receiving" or "querying"
those are                           % phrase see if "those X are" is clearer?
design is motivated                 % phrase "inspired by" is probably better than "motivated" for design
locations throughout the world      % phrase drop "throughout the world"
e.g., as opposed to                 % phrase if you're giving examples, you're not talking about what isn't.  drop "e.g."
in addition, we also                % phrase remove either "also" or "in addition"
other related issues                % phrase probably remove "other"
the aforementioned                  % phrase "these xs" or "this x" would be less snooty
center around                       % phrase (cook) a center is a point: "center on" is okay.
could care less                     % phrase (cook) 'really? how much less could you care?' (should be couldn't)
grouped together                    % phrase redundant.  "grouped" alone should suffice.
put together                        % phrase long: "construct" "build" or "assemble"
consistent with each other          % phrase redundant.  "consistent" suffices.
be accomplished with                % phrase try "requires" "uses" "needs"?
the lack of knowledge of            % phrase would "X is unknown" work better?
gets to know                        % phrase you mean "learns"
trying to look like                 % phrase you mean "acting", "emulating", or "mimicing"
has got to be                       % phrase "must be"
got                                 % phrase try "became" "received" ?
gotten                              % phrase try "helped" ?
live in a vacuum                    % phrase a tired metaphor that makes me want to vomit.
positive impact                     % phrase try "benefit"
negative impact                     % phrase try "harm" or "consequences"
adverse impact                      % phrase try "harm" or "consequences"
adversely impacting                 % phrase try "harming" or "hurting"
discuss the issues of               % phrase could probably drop "the issues of" unless there's a list
the presence of                     % phrase not far from 'is', 'has', etc.
does not allow                      % phrase consider "forbids" or "prohibits"
and/or                              % phrase just say or.
there is the potential to           % phrase just say may.
there is the possibility that       % phrase just say might.
can be achieved                     % phrase maybe not so good?
find out                            % phrase perhaps determine?
in the absence of                   % phrase perhaps without?
in the presence of                  % phrase perhaps with?
set up                              % phrase perhaps create, configure, or initialize
in the face of                      % phrase can be overused.  try despite?
several times (at|of)               % phrase discouraged by Kurt.
a large degree of                   % phrase ick.
we start by first                   % phrase redundant. ("first, we" or "we start by").
in general, they are usually        % phrase redundant.
refers to the notion                % phrase define your term precisely if possible.
a significant amount of             % phrase probably just "significant"
real practical                      % phrase as opposed to imaginary practical?
people that are                     % phrase use people who are?
additional detail that we add       % phrase as opposed to additional detail that we subtract?
in some cases and not in others     % phrase "in some cases"
it is known that                    % phrase just say it.
caused due to                       % phrase "caused by"
a result of the fact that           % phrase "caused by"
results (indicate|show|suggest)     % phrase drop
research (indicates|show|suggest)   % phrase drop
can be attributed to the fact that  % phrase "is because"
a large set of                      % phrase probably don't care that it is a set.
a small set of                      % phrase probably don't care that it is a set: use 'a few'
provides a look at                  % phrase (timid) probably mean "shows".
in most cases                       % phrase "usually"
continue into the forseeable future % phrase "continue".
for the forseeable future           % phrase drop.
fail to successfully                % phrase "fail to" is sufficient.
Clearly,                            % syntax starting a sentence with clearly confuses me.
in different continents             % phrase ON different continents, IN different countries
(we|to) handle                      % phrase use a more specific verb like address, treat, solve
handling                            % phrase use a more specific verb like addressing, treating, solving, mitigating (unless handling errors or exceptions)
For the purposes of                 % phrase "For"
We observe that                     % phrase drop.
some degree of                      % phrase "some"
in the problem of                   % phrase (contributed by rap)
conclude several things             % phrase make (draw) several conclusions
extra bonus                         % phrase "bonus"
added bonus                         % phrase "bonus"
it is important to emphasize that   % phrase use diction to emphasize.
it is possible that                 % phrase "x may y"
caused due to                       % phrase "caused by"
recent work by                      % phrase could maybe be dropped, as the cite will include the date.
identify the location of            % phrase "find"
that go across                      % phrase "that cross"
ideally, we would like              % phrase "we would like"
enabling the ability to             % phrase "supporting" or "allowing" or "permitting"
absolutely essential                % phrase essential is.
we essentially do                   % phrase essentially is a poor adverb.  "The essence of our algorithm is a..."
Essentially,                        % phrase maybe "In essence," but could also be removed.
In this section (we|I)              % phrase "In this section, we", or "In this section, I"
essentially all                     % phrase "most"
past experience                     % phrase "experience" http://www.cmu.edu/styleguide/trickywords.html
particulary difficult primarily     % phrase simplify
intuition about why                 % phrase "intuition as to why"
Recall from above                   % phrase "recall"
Further, (I|we) will also           % phrase drop further or also
respectively                        % phrase unneeded.
in terms of                         % phrase don't need this.
the extent to which                 % phrase "how much"
make sure                           % phrase "ensure"
make up                             % phrase "constitute" "compose"
make use of                         % phrase "use"
make a decision                     % phrase "decide"
make a guess                        % phrase "guess"
since that time                     % phrase "since then"
choices to make                     % phrase "choices"
certain limitations                 % phrase what does 'certain' add to limitations?
will [a-z]* in the future           % phrase "will"
business entities                   % phrase "businesses"
rely primarily on                   % phrase "primarily" weakens "rely".  perhaps just "use" would be simpler.
has the potential to                % phrase can
have not yet developed              % phrase "have yet to develop"
to be effective,                    % phrase probably redundant.
provide information about           % phrase "tell how" "reveal" "expose" "disclose"
are different,                      % phrase "differ"
have already been                   % phrase "have been"? "were"?
as appropriate                      % phrase not needed?
only rarely                         % phrase "rarely" is probably enough.
is effective at                     % phrase "can"
foremost among them is              % phrase "foremost is" would be shorter.
those that have no                  % phrase those without
that have no                        % phrase "without"?
a variety of diverse                % phrase redundant
be highly valuable in               % phrase simplify.
the overall goal                    % phrase 'the goal'
sometimes an? [a-z]+ will           % phrase an x may
this is perhaps because             % phrase this may be because
adding an additional                % phrase redundant
IP protocol                         % phrase redundant
works well                          % phrase be more specific.
something                           % phrase could eliminate.
to keep from                        % phrase "to avoid"
[\.,] since (!then)                 % phrase probably you mean "because" unless you're talking about time. -- "has since" is okay.
performance characteristics         % phrase rare that characteristics adds.
takes into account                  % phrase considers
specify particular                  % phrase if specifying, particular should be redundant.
prototype implementation            % phrase "implementation" is redundant.
given a particular                  % phrase "given a" is probably enough
described in detail (in|below)      % phrase use "detailed"
relatively more                     % phrase more is already relative.
focus primarily on                  % phrase bad metaphor: subject of focus is singular.
primary focus                       % phrase bad metaphor: subject of focus is singular.
relatively more                     % phrase more is already relative.
gives [a-z]+ [a-z]+ information about % phrase use "tells" x
gives [a-z]+ information about      % phrase use "tells" x
an important question to ask is     % phrase just ask it.
an interesting thing                % phrase avoid saying something is interesting.  if you have to say it, it isn't.
checks to see if                    % phrase "checks" or "determines"
have an effect on                   % phrase "affect"
an important question to ask is     % phrase just ask it.
an interesting thing                % phrase avoid saying something is interesting.  if you have to say it, it isn't.
checks to see if                    % phrase "checks" or "determines"
we can see                          % phrase "we can see" isn't formal enough.
still remain                        % phrase "remain".
change over time                    % phrase "change"
turn into                           % phrase "become"
looking back in retrospect          % phrase pick.
ensures that there will be no       % phrase "prevents"
does have                           % phrase "has"
first step toward this              % phrase "toward this" can probably be dropped.
can potentially be                  % phrase "might be", or just "can be"
obviates the need for               % phrase just obviates x, not obviates the need for x.
it is indeed                        % phrase "it is", though still passive.
planning in advance                 % phrase when else might you plan?
a lot of                            % phrase "many"
keep in mind                        % phrase "consider" (or drop)
it is clear that                    % phrase if clear, you don't have to say it.
especially true                     % phrase true is an absolute, can't be especially true.
making it increasingly difficult    % phrase preventing, discouraging, impeding, blocking, slowing...
is potentially                      % phrase "may be"
have been [a-z]* in the past        % phrase 'in the past' is redundant with tense.
amount of time  % phrase "duration"
should ideally % phrase "should"
are of great benefit to % phrase "help" or "aid"
are of benefit to % phrase "help" or "aid" or "promote"
important here % phrase consider "relevant"
while at the same time % phrase "while" is enough.
are able to % phrase can
subvert the proper operation of % phrase subvert
speed slow % phrase speed is probably redundant.
of size no smaller than % phrase "of size" is probably redundant
of size no larger than % phrase "of size" is probably redundant
of size smaller than % phrase "of size" is probably redundant
of size larger than % phrase "of size" is probably redundant
might potentially % phrase "might"
in the context of % phrase "in" avoid, if possible.
increase the amount of % phrase probably just increase.
show the difference between % phrase compare
in addition, we also % phrase pick.
overhead efficiency % phrase huh?
have an effect on % phrase "affect"
have a signficant effect on %  phrase "affect"
we find % phrase can usually be removed
this suggests % phrase remove or make more precise
effective for providing	   	 % phrase remove
we performed a                   % phrase just use the verb directly
we perform a                     % phrase just use the verb directly
were able to                     % phrase could
are able to                      % phrase can


==> style/tricks.tex <==

 
% this is where we disable/enable the note
\newif\ifnotes
\notestrue % turn this on and disable the next line to display notes
% \notesfalse % turn this on to hide notes, which overwrites the previous line. 
 
\definecolor{fycolor}{HTML}{c378e3} % fumeng's color
\newcommand{\fy}[1]{\ifnotes{\leavevmode{\color{fycolor}{(Fumeng: #1)}}}\fi}
\newcommand{\fyedit}[1]{\ifnotes{\leavevmode\color{fycolor}{#1}}\elseif{#1}\fi}
\newcommand{\fyreplace}[2]{\ifnotes{\color{fycolor}{\sout{#1} {#2}}}\else{#2}\fi}
\newcommand{\fydelete}[1]{\ifnotes{\color{fycolor}{\sout{#1}}}\fi}
\newcommand{\fyadd}[1]{\ifnotes{\color{fycolor}{#1}}\else{#1}\fi}
% \newcommand{\todo}[1]{\ifnotes{\leavevmode\color{red}{#1}}\fi}
